Density-aware Chamfer Distance as a Comprehensive Metric for Point Cloud Completion

Chamfer Distance (CD) and Earth Mover's Distance (EMD) are two broadly adopted metrics for measuring the similarity between two point sets. However, CD is usually insensitive to mismatched local density, and EMD is usually dominated by global distribution while overlooks the fidelity of detailed structures. Besides, their unbounded value range induces a heavy influence from the outliers. These defects prevent them from providing a consistent evaluation. To tackle these problems, we propose a new similarity measure named Density-aware Chamfer Distance (DCD). It is derived from CD and benefits from several desirable properties: 1) it can detect disparity of density distributions and is thus a more intensive measure of similarity compared to CD; 2) it is stricter with detailed structures and significantly more computationally efficient than EMD; 3) the bounded value range encourages a more stable and reasonable evaluation over the whole test set. We adopt DCD to evaluate the point cloud completion task, where experimental results show that DCD pays attention to both the overall structure and local geometric details and provides a more reliable evaluation even when CD and EMD contradict each other. We can also use DCD as the training loss, which outperforms the same model trained with CD loss on all three metrics. In addition, we propose a novel point discriminator module that estimates the priority for another guided down-sampling step, and it achieves noticeable improvements under DCD together with competitive results for both CD and EMD. We hope our work could pave the way for a more comprehensive and practical point cloud similarity evaluation. Our code will be available at: https://github.com/wutong16/Density_aware_Chamfer_Distance .

==> articles/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See supplementary material.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We will release the code upon the paper accepted.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Sec.~\ref{sec:experiment}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Sec.~\ref{sec:experiment}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{MVP dataset~\cite{pan2021variational}.}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> deprecated/formulation.tex <==
% !TEX root = ../main.tex
\section{Formulation}
\label{sec:formulation}
\subsection{Deduction and Interpretation}
Chamfer Distance is one of the most widely used metrics to evaluate the \needcheck{distance between two shapes}, and it is defined as: 
\begin{equation}
    CD(S_1, S_2) = \frac{1}{|S_1|}\sum_{x\in S_1}\min_{y\in S_2}||x-y||_2 + \frac{1}{|S_2|}\sum_{y \in S_2}\min_{x\in S_1}||y-x||_2.
\end{equation}
The clean and effective formulation promotes stable and consistent evaluations between topologies with relatively uniform and similar distributions.
However, as could also be observed in Fig.~\missref{teaser}, it still suffers from several cases by nature as follows:
\textbf{1)} the square operation makes it sensitive to outliers though these points may not necessarily induce tremendous violation to the overall topology; 
and \textbf{2)}, the nearest point query operation makes it less sensitive to the issue of imbalanced distribution, and uneven importance of each point in the set.

% * forward deduction *
Therefore, based on the original formulation, we aim to propose a new metric that preserves the capacity of similarity evaluation while alleviating the problems above at the same time.
Firstly, in order to set up a boundary to paired point-wise distance, we leverage the mathematical approximation that $\lim_{z\to 0}e^z = z + 1$ and take $z = -||x-y||_2$. Because of the [0,1] normalization and top-1 nearest neighbouring operation, the condition where $z \approx 0 $ would be easily matched, and thus we have:
\begin{equation}
    \begin{aligned}
    d_{CD}(S_1, S_2) \approx \frac{1}{|S_1|}\sum_{x\in S_1}\min_{y\in S_2}(1 - e^{-||x-y||_2}) + 
    \frac{1}{|S_2|}\sum_{y\in S_2}\min_{x\in S_1}(1 - e^{-||y-x||_2}). \\ 
    \end{aligned}
    \label{eq:metric_d1}
\end{equation}
Thanks to the property of the exponential function $e^{-z}(z>0)$, each point-wise distance is mapped to a value between [0,1]. As a result, the formulation also lies a natural boundary of [0,1] to the overall shape distance. Although the approximation would be less accurate as the point-wise distance gets away from zero, it exactly helps to eliminate the sensitivity of the outliers by suppressing the square growth to a constant. We could add another scale factor $\alpha$ as in Eqn.~\ref{eq:metric} to adjust the sensitivity. 
% todo: 'sensitivity' appears too many times, change to synonym
% todo: shall we add some lemmas here?

Secondly, as for the issue of imbalance, we denote that the ambiguity of CD is partially due to the fact that the points in the same set are not of 'equal importance'. 
To be specific, assume $S_1$ to be a uniform point cloud and $S_2$ an inhomogeneous one; consider two points $y_1, y_2 \in S_2$ with $y_1$ locating at a sparse area of the shape surface and $y_2$ in a relatively dense area. 
The calculation of $CD(S_1,S_2)$ would likely get $y_1$ frequently queried to be the nearest neighbour by points in $S_1$ due to the local sparsity; while the case for $y_2$ could be exactly the opposite: seldom or probably zero points in $S_1$ would view it as their nearest neighbour. This leads to uneven influence of each point to the evaluation results.

% todo: define the single word 'query' to be 'view as the nearest neighbour' somewhere proper.
Further more, assume that $n_{y_1}$ points in $S_1$ queries $y_1$, while each of them is unaware of neither the others nor the total querying times $n_{y_1}$; in other words, the existence of $y1$ blocks $x$ from sensitively perceiving the real distribution around it, and the contribution of $y_1$ to each $x$ is not eliminated even though it is being shared. 
This unreasonable case reveals the reason why CD is not sensitive to imbalanced distribution, which is another important factor on evaluating point cloud quality.

We denote that the overall contribution of each points to the evaluation system shell be normalized, thus $\frac{1}{n_y}$ is introduced to deal with the case where $y$ is being shared by multiple $x$s.
\begin{equation}
    \begin{aligned}
    d_{BCD}(S_1, S_2) &= \frac{1}{|S_1|}\sum_{x\in S_1} \left(1 - \frac{1}{n_{\hat{y}}}e^{-\alpha||x-\hat{y}||_2}\right) + 
    \frac{1}{|S_2|}\sum_{y\in S_2} \left(1 - \frac{1}{n_{\hat{x}}}e^{-\alpha||y-\hat{x}||_2}\right),
    \end{aligned}
    \label{eq:metric}
\end{equation}
% todo: this is for equal point number, and would be extended to inequal number later
where $\hat{y} = \min_{y\in S_2}||x-y||_2, \hat{x} = \min_{x\in S_1}||y-x||_2$, and $n_y$ is the query times of point $y$.
% * backward interpretation *
We then take a closer look at Eqn.~\ref{eq:metric} and further interpret its properties from \needcheck{the manner of energy (bushi}, taking the first term as an example without loss of generality. 
% haven't thought of a good presentation, but I do think this part shares some relationship with energy model.

We begin with the single system $S_1$ with no $S_2$ provided, then the distance from each points $x$ could be viewed as infinity, and overall metric value of the system achieves its upper bound of 1.
Then given $S_2$, for each $x \in S_1$, its contribution to the metric value could be $E^{12}(x)$ in Eqn.~\ref{eq:energy}, and the contribution of each $y \in S_2$ could be $E^{12}(y) \in [-1,0]$:
\begin{equation}
  E^{12}(x) = \frac{1}{|S_1|}\min_{y\in S_2}(1 - e^{-||x-y||_2})\in [0,1], \ \
  E^{12}(y) = - \frac{1}{n_{y}} \sum_{x \in \hat{S}_{n_y}} e^{-||x-y||_2} \in [-1,0]
  \label{eq:energy}
\end{equation}

\subsection{Comparison with EMD}
The deduction above starts from the formulation of CD and targets at addressing two drawbacks of it. Below we would further discuss the difference with other metrics.
\noindent\textbf{Comparison with EMD}
As shown in Fig.~\ref{fig:teaser}, the distributions of BCD and EMD in the noise-imbalance evaluation matrix are relatively similar, which aligns well with our goal that the new metric preserves the good properties of EMD and prefers both distributional balance and shape similarity. 
However, we also empirically observed that EMD is sometimes \textit{dominated} by the global distribution, which weankens the influence of local structure fidelity before a satisfying global balance being preserved. As shown in Fig.~\missref{}

\begin{equation}
    d_{EMD}(S_1, S_2) = \min\limits_{\phi:S_1\rightarrow S_2}\sum\limits_{x\in S_1}||x - \phi(x)||_2.
\end{equation}


\noindent\textbf{Computational Properties}
One of the In particular, it had been shown that
the practical computational efficiency of EMD is at the order
of max{|P|, |Q|}3 [33], which can be expensive. There is
a recent line of work using entropic version of EMD or in % general Wasserstein distancesto speed up the computation of EMD.
1) EMD needs one-to-one mapping, and n

\noindent\textbf{Any metric that evaluates the uniformalty of point cloud? }
Espescially in up-sampling.
\noindent\textbf{}
% 1) Table and several cases to compare them
% 2) analysis of EMD and New Metric 
% 5) the problem of CD can be visualized (importance map)
% 6) this is important: think of how we statistic the results to show it aligned with EMD.
% 7) change temperature to adjust the value range, currently too small
% 8) global imbalance and local less uniform


==> deprecated/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> deprecated/methodology.tex <==
% !TEX root = ../main.tex
\section{Methodology}

% words that appear too many times: specifically, preserve
In this section, we take the task of point cloud completion as an example to analyze how the previously mentioned properties affect the network training and inference process in Sec.~\ref{sec:two_stage}. 
We also propose a simple yet effective extension to the two-stage completion framework in Sec.~\ref{sec:our_method} to address these problems.

\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/framework.pdf}
	\caption{\small
	Two-stage framework; mean shape study in the first stage; up-sampling and guided down-sampling in the second stage.
	}
	\label{fig:framework}
\end{figure}

\subsection{Two-Stage Completion Pipeline}
\label{sec:two_stage}
The two-stage coarse-to-fine completion pipeline was first proposed by PCN~\cite{yuan2018pcn} and further improved by a number of its following works~\misscite{}. Specifically, the procedure involves the generation of a low-resolution coarse shape based on a global feature followed by a refinement stage with more points and enhanced details.
% We denote that this framework trained with CD loss could suffer from two types of imbalance issue, between the structure and details, seen and unseen regions, respectively. 
% We adopt the recent VRC~\cite{pan2021variational} framework as the baseline model, would like to start from the widely used two-stage 

\noindent\textbf{Coarse Shape Generation}
% Despite the issues discussed in Sec.~\ref{sec:formulation}, CD is still one of the most popular and effective loss functions for many point cloud related tasks.
Given a partial point cloud as input, a global feature is extracted by a PointNet-like MLP network and then a decoder generate a sparse and coarse point cloud $p_0$ accordingly.
Though $p_0$ maintains a relatively reasonable global shape, it usually fails to capture and depict detailed structures of the input.
% The reason from a high-level perspective is that a single global vector is not representative enough~\misscite{} to save all the ,
% while we also provide another low-level explanation based on the 
Although CD loss does not involve any hard assignment between prediction and ground truth point sets, it is observed that the output coordinates from each position of the last fully connected layer of the decoder has a relatively convergent local distribution.
Consider them to be under Gaussian distribution, We calculate and visualize the mean and variance for each category across the test set as shown in Fig.~\missref{}. 
Thanks to the inherent distribution that it usually keeps a complete structure, but an obvious imbalance of density and variance can also be observed among different parts according to how commonly they are shared across the dataset. 
This problem exists for the mean shape and most instances in the test set, and shell be handled in the second stage.

\noindent\textbf{Detail Preserved Refinement}
Upon obtaining the low-resolution coarse shape, the refining stage aims to 1) precisely reconstruct the input point cloud without loss of details and to 2) improve the quality of coarse shape especially for the unseen part, hopefully transferring some shared structure details from the seen part to it.
One tricky thing is that, the first few properly located points in an unseen area significantly reduces the CD loss, while the gain soon decays with more points predicted there. Considering the side effect that inaccurate points would bring in extra corruption to the overall distance measurement by CD, lying more points in the seen region with high-confidence usually boosts the CD performance while hurting the distribution at the same time.

\subsection{Up-sampling and Guided down-sampling}
\label{sec:our_method}
One natural idea to alleviate imbalance is to first up-sample the point cloud then down-sample via Furthest Point Sampling (FPS). 
However, FPS naturally select more points from sparse area, which increases the risk of including more outliers, resulting in significantly lower EMD at the sacrifice of CD.
As a result, we aim to count for the matters of both imbalance and outliers during the sampling process.

We train a network to predict the privilege of selecting each point. 
The predictor has an MLP structure and takes the local feature and point coordinates as input and predict $z$ as a regression problem:
\begin{equation}
h(f_x, x) = \left\{
\begin{aligned}
& \log_2(n)  & n_x > 0 \\
& d(x, P_{gt}) * \alpha  & n_x = 0.
\end{aligned}
\right.
\end{equation}

Then at inference time, we randomly sample from the refined point cloud based on the point-wise probability:
\begin{equation}
    p = \log{- \beta * z + \gamma},
\end{equation}
before performing FPS and get the final down-sampled points. 
This process could effectively reduce CD, as to be shown in Sec.~\missref{}.
What is worth noting is that, adopting EMD as the training loss would also significantly promotes the uniformity and suppresses the EMD metric, while the details and structures are not decently retained as to be shown in Fig.~\ref{fig:comparison}, resulting in a relatively high CD loss at the same time.

==> tables/bcd_loss.tex <==
% Table generated by Excel2LaTeX from sheet 'DaCD_loss'
\begin{table}[htbp]
  \centering
  \small
  \caption{Evaluation results by different metrics when trained on each of them. * denotes that we apply $L_{EMD}$ only on the final output and intermediate results with \textit{less} points are supervised by $L_{CD}$.}
    \begin{tabular}{c|ccc|ccc}
    \toprule
    \toprule
    \small
    Model & \multicolumn{3}{c|}{PCN~\citep{yuan2018pcn}} & \multicolumn{3}{c}{VRC~\citep{pan2021variational}} \\
    \midrule
    \small
    Metric / Loss & $L_{CD}$ & $ L^*_{EMD}$ & $L_{DCD}$ & $L_{CD}$ & $L^*_{EMD}$ & $L_{DCD}$ \\
    \midrule
    $CD$ & 9.78  & 10.70 & \textbf{9.36} & 6.09  & 7.87  & \textbf{5.85} \\
    \textbf{$EMD$} & 6.80  & \textbf{3.97} & 4.71  & 5.27  & \textbf{3.62} & 5.14 \\
    \textbf{$DCD$} & 0.553 & 0.537 & \textbf{0.526} & 0.462 & 0.461 & \textbf{0.457} \\
    \bottomrule
    \bottomrule
    \end{tabular}%
  \label{tab:dacd_loss}%
\end{table}%

